Optimizing Polymatroid Functions

We consider a class of optimization problems that involve determining the maximum value that a function in a particular class can attain subject to a collection of difference constraints. We show that a particular linear programming technique, based on duality and projections, can be used to rederive some structural results that were previously established using more ad hoc methods. We then show that this technique can be used to obtain a polynomial-time algorithm for a certain type of simple difference constraints. Finally we give lower bound results that show that certain possible extensions of these results are probably not feasible.

==> macros.tex <==
%\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}

% the following is to allow eqnarray to run from one page to another
%\let\endproof\relax
%\let\proof\relax
%\input{macros}

%%% ==== Packages
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{cite}
\usepackage{fullpage}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{tikz,tikz-qtree,tikz-qtree-compat}
\usetikzlibrary{shapes,decorations,arrows,calc,fit}
%\usepackage{fancyheadings}
\usepackage{color,xspace,colortbl}
\usepackage{float}
\usepackage[ruled]{algorithm2e}
\usepackage[noend]{algpseudocode}
\usepackage{enumitem}
\usepackage{balance}
\usepackage{todonotes}
\usepackage{url}
\usepackage{multirow}

\colorlet{LightViolet}{violet!40}
\colorlet{LightRed}{red!40}
\colorlet{LightOrange}{orange!40}
\colorlet{LightGreen}{green!40}
\colorlet{LightBlue}{blue!40}
\colorlet{DarkGreen}{green!50!black}
\colorlet{DarkRed}{red!70!black}
\colorlet{DarkCyan}{red!70!black}
\colorlet{DarkBlue}{blue!80!black}
\definecolor{DarkOrange}{rgb}{1.0, 0.49, 0.0}
\definecolor{Airforceblue}{rgb}{0.36, 0.54, 0.66}
\newcommand{\Note}[1]{{\color{DarkRed} #1}}
\newcommand{\Bigstar}{\mathop{\bigstar}}
\newcommand{\Airforceblue}[1]{{\color{Airforceblue} #1}}
\newcommand{\DarkBlue}[1]{{\color{DarkBlue} #1}}
\newcommand{\LightBlue}[1]{{\color{LightBlue} #1}}
\newcommand{\DarkOrange}[1]{{\color{DarkOrange} #1}}
\newcommand{\LightOrange}[1]{{\color{LightOrange} #1}}
\newcommand{\LightRed}[1]{{\color{LightRed} #1}}
\newcommand{\DarkGreen}[1]{{\color{DarkGreen} #1}}
\newcommand{\Emphasize}[1]{{\color{DarkGreen} #1}}

%%% ==== Misc macros, specific to this paper
\newcommand{\yell}[1]{{\color{red} \textbf{#1}}}
\newcommand{\ayell}[1]{{\color{green} {#1}}}
\newcommand{\hqn}[1]{\todo[inline,color=cyan]{\textsf{#1} \hfill \textsc{--Hung.}}}
\newcommand{\xln}[1]{\todo[inline,color=green]{\textsf{#1} \hfill \textsc{--Long.}}}
\newcommand{\dan}[1]{\todo[inline,color=yellow]{\textsf{#1} \hfill \textsc{--Dan.}}}
\newcommand{\mak}[1]{\todo[inline,color=orange]{\textsf{#1} \hfill \textsc{--Mahmoud.}}}
\newcommand{\nop}[1]{}

\newcommand{\heavy}{\text{\sf heavy}}
\newcommand{\light}{\text{\sf light}}
\newcommand{\fecp}{\text{\sf FECP}}
\newcommand{\poly}{\text{\sf poly}}
\newcommand{\dc}{\text{\sf DC}}
\newcommand{\cc}{\text{\sf CC}}
\newcommand{\fd}{\text{\sf FD}}
\newcommand{\FD}{\text{\sf FD}}
\newcommand{\hdc}{\text{\sf HDC}}
\newcommand{\vietnam}{\text{\sf vietnam}}
\newcommand{\saigon}{\text{\sf saigon}}
\newcommand{\hanoi}{\text{\sf hanoi}}
\newcommand{\germany}{\text{\sf germany}}
\newcommand{\england}{\text{\sf england}}
\newcommand{\usa}{\text{\sf usa}}
\newcommand{\fall}{\text{\sf fall}}
\newcommand{\winter}{\text{\sf winter}}
\newcommand{\incomp}{\perp}
\newcommand{\flow}{{\sf inflow}}

\newcommand{\Assumption}{Conditional query assumption\xspace}
\newcommand{\ProdMar}{Product-marginalization assumption\xspace}
\newcommand{\conQuery}{conditional query\xspace}
\newcommand{\conQueries}{conditional queries\xspace}
\newcommand{\LW}{\mathsf{LW}}
\newcommand{\elf}{\mathsf{ELF}}
\newcommand{\fkagm}{\text{\sc FK-AGM}}
\newcommand{\FKAGM}{\text{{\sf FK-AGM}}}
\newcommand{\LB}{\text{{\sf LogicBlox}}}
\newcommand{\lftj}{\text{{\sf LFTJ}}}
\newcommand{\gj}{\text{{\sf Generic-Join}}}
\newcommand{\faqcs}{\text{\sf FAQ-SS}}
\newcommand{\fdb}{\text{\sf FDB}}
\newcommand{\bcp}{\text{\sf BCP}}
\newcommand{\faq}{\text{\sf FAQ}}
\newcommand{\csma}{\text{\sf CSMA}}
\newcommand{\panda}{\text{\sf PANDA}}
\newcommand{\qfbcq}{\text{\sf QFBCP}}
\newcommand{\twister}{\text{\sf Twister}}
%\newcommand{\cqe}{\text{\sf CQE}}
\newcommand{\parents}{\text{parents}}

%%% ==== Complexity classes
\newcommand{\complexityclass}{\mathbf}
\newcommand{\sharpP}{\#\complexityclass{P}}
\newcommand{\acc}{\complexityclass{ACC}}
\newcommand{\np}{\complexityclass{NP}}
\newcommand{\logspace}{\complexityclass{LOGSPACE}}
\newcommand{\nlogspace}{\complexityclass{NLOGSPACE}}
\newcommand{\pspace}{\complexityclass{PSPACE}}
\newcommand{\fo}{\complexityclass{FO}}
\newcommand{\fpt}{\complexityclass{FPT}}
\newcommand{\wone}{\complexityclass{W}[1]}
\newcommand{\W}{\complexityclass{W}}
\newcommand{\rp}{\complexityclass{RP}}
\newcommand{\corp}{\complexityclass{coRP}}
\newcommand{\p}{\complexityclass{P}}
\newcommand{\nexp}{\complexityclass{NEXP}}
\newcommand{\pcp}{\complexityclass{PCP}}

%%% ==== Function names
\newcommand{\functionname}[1]{\text{\sf #1}}

\newcommand{\Idem}{\functionname{Idem}}
\newcommand{\tw}{\functionname{tw}}
\newcommand{\Ftw}{\functionname{$F$-p-tw}}
\newcommand{\Ffhtw}{\functionname{$F$-p-fhtw}}
\newcommand{\faqw}{\functionname{faqw}}
\newcommand{\Fhtw}{\functionname{$F$-p-htw}}

\newcommand{\FFtw}{\functionname{$F$-free-tw}}
\newcommand{\FFfhtw}{\functionname{$F$-free-fhtw}}
\newcommand{\FFhtw}{\functionname{$F$-free-htw}}

\newcommand{\Lss}{\functionname{$L$-ss}}
\newcommand{\Fss}{\functionname{$F$-ss}}
\newcommand{\htw}{\functionname{htw}}
\newcommand{\fhtw}{\functionname{fhtw}}
\newcommand{\adw}{\functionname{adw}}
\newcommand{\atoms}{\functionname{atoms}}
\newcommand{\dom}{\functionname{Dom}}
\newcommand{\vars}{\functionname{vars}}
\newcommand{\free}{\functionname{free}}
\newcommand{\arity}{\functionname{arity}}
\newcommand{\weight}{\functionname{weight}}
\newcommand{\clr}{\functionname{color}}
\newcommand{\wcoj}{\functionname{WCOJ}}

\newcommand{\true}{\functionname{true}}
\newcommand{\false}{\functionname{false}}
\newcommand{\nan}{\functionname{NaN}}

\newcommand{\InsideOut}{\functionname{InsideOut}}
\newcommand{\basicOI}{\functionname{Recursive-OutsideIn}}
\newcommand{\iterativeOI}{\functionname{Iterative-OutsideIn}}
\newcommand{\OI}{\functionname{OutsideIn}}

\newcommand{\avg}{\functionname{avg}}
\newcommand{\unique}{\functionname{unique}}
\newcommand{\xor}{\functionname{XOR}}

%%% ==== Problem names
\newcommand{\problemname}[1]{\text{\sf #1}}
\newcommand{\mcm}{\problemname{MCM}}
\newcommand{\uniqueclique}{\problemname{Unique-Clique}}
\newcommand{\uniquekclique}{\problemname{Unique-$k$-Clique}}
\newcommand{\sumprod}{\problemname{Sum-Product}}
\newcommand{\maxprod}{\problemname{Max-Product}}
\newcommand{\csp}{\problemname{CSP}}
\newcommand{\pgm}{\problemname{PGM}}
\newcommand{\cqe}{\problemname{CQE}}
\newcommand{\bcq}{\problemname{BCQ}}
\newcommand{\sat}{\problemname{SAT}}
\newcommand{\ssat}{\problemname{\#SAT}}
\newcommand{\wssat}{\problemname{\#WSAT}}
\newcommand{\scsp}{\problemname{\#CSP}}
\newcommand{\scq}{\problemname{\#CQ}}
\newcommand{\sqcq}{\problemname{\#QCQ}}
\newcommand{\mpf}{\problemname{MPF}}
\newcommand{\FFT}{\problemname{FFT}}
\newcommand{\EVO}{\problemname{EVO}}
\newcommand{\LE}{\problemname{LinEx}}
\newcommand{\CW}{\problemname{CW}}
\newcommand{\CWE}{\problemname{CWE}}
\newcommand{\qcq}{\problemname{QCQ}}
\newcommand{\sacq}{\problemname{\#ACQ}}
\newcommand{\cq}{\problemname{CQ}}


%%% ==== Algorithms
\newcommand{\nprr}{\text{\sf NPRR}\xspace}
\newcommand{\leapfrog}{\text{\sf Leapfrog-Triejoin}\xspace}
\newcommand{\agm}{\text{\sf AGM}\xspace}
\newcommand{\fama}{\text{\sf FaMa}}
\newcommand{\pr}{\mathbb P}
\newcommand{\supp}{\text{\sf supp}}
\newcommand{\lr}{\text{\sf LR}}
\newcommand{\tetris}{\text{\sf Tetris}\xspace}

\newcommand{\sku}{\textsf{s}}
\newcommand{\town}{\textsf{t}}
\newcommand{\week}{\textsf{w}}
\newcommand{\district}{\textsf{d}}
\newcommand{\Sales}{\textsf{sales}}
\newcommand{\Sku}{\textsf{sku}}
\newcommand{\Store}{\textsf{Store}}
\newcommand{\City}{\textsf{city}}
\newcommand{\Country}{\textsf{country}}
\newcommand{\Town}{\textsf{town}}
\newcommand{\Week}{\textsf{week}}
\newcommand{\District}{\textsf{district}}

%%% ==== Common Abbreviations
\newcommand{\calA}{\mathcal A}
\newcommand{\calR}{\mathcal R}
\newcommand{\calL}{\mathcal L}
\newcommand{\calT}{\mathcal T}
\newcommand{\calP}{\mathcal P}
\newcommand{\calX}{\mathcal X}
\newcommand{\calY}{\mathcal Y}
\newcommand{\calB}{\mathcal B}
\newcommand{\calC}{\mathcal C}
\newcommand{\calD}{\mathcal D}
\newcommand{\calE}{\mathcal E}
\newcommand{\calF}{\mathcal F}
\newcommand{\calG}{\mathcal G}
\newcommand{\calH}{\mathcal H}
\newcommand{\calV}{\mathcal V}
\newcommand{\calU}{\mathcal U}

\newcommand{\F}{\mathbb F} % a field
\newcommand{\Z}{\mathbb Z} % integers
\newcommand{\N}{\mathbb N} % the natural numbers
\newcommand{\R}{\mathbb R} % the real numbers
\newcommand{\D}{\mathbf D} % bold-face D, used for generic domain
\newcommand{\Q}{\mathbb Q} % the real numbers
\newcommand{\Mod}{\text{\sf M}}
\newcommand{\Nor}{\text{\sf N}}
\newcommand{\sa}{\text{\sf SA}}


\newcommand{\perm}{\text{perm}}

\newcommand{\stab}{\textnormal{\sc stab}}
\newcommand{\infl}{\textnormal{\sc inf}}
\newcommand{\func}[1]{\textnormal{\sc #1}}

\newcommand{\la}{\leftarrow}
\newcommand{\ra}{\rightarrow}

\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}}
\newcommand{\grad}[1]{\gv{\nabla} #1} % for gradient
\newcommand{\pd}[2]{\frac{\partial#1}{\partial#2}}




\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
%\newcommand{\argmax}{\text{argmax}}

\newcommand{\threesum}{\text{$3$-{\sf SUM}}}
%\newcommand{\pr}{\mathop{\textnormal{Prob}}}
\newcommand{\E}{\mathbb E}

%%% ==== Common shortcuts
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\bp}{\begin{proof}}
\newcommand{\ep}{\end{proof}}
\newcommand{\bcor}{\begin{cor}}
\newcommand{\ecor}{\end{cor}}
\newcommand{\bthm}{\begin{thm}}
\newcommand{\ethm}{\end{thm}}
\newcommand{\blmm}{\begin{lmm}}
\newcommand{\elmm}{\end{lmm}}
\newcommand{\bdefn}{\begin{defn}}
\newcommand{\edefn}{\end{defn}}
\newcommand{\bprop}{\begin{prop}}
\newcommand{\eprop}{\end{prop}}
\newcommand{\bconj}{\begin{conj}}
\newcommand{\econj}{\end{conj}}
\newcommand{\bopm}{\begin{opm}}
\newcommand{\eopm}{\end{opm}}
\newcommand{\brmk}{\begin{rmk}}
\newcommand{\ermk}{\end{rmk}}

\newcommand{\qnom}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}

\newcommand{\sto}{\textnormal{subject to}}

\newcommand{\norm}[1]{\left\|#1\right\|}

\newcommand{\suchthat}{\ | \ }
\newcommand{\inner}[1]{\left\langle #1 \right\rangle}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\vol}[1]{\mathop{\textnormal{Vol}} #1}
\newcommand{\var}[1]{\mathop{\textnormal{Var}}\left[#1\right]}
\newcommand{\cov}[1]{\mathop{\textnormal{Cov}}\left[#1\right]}
\newcommand{\per}[1]{\mathop{\textnormal{per}} #1}
\newcommand{\trace}[1]{\mathop{\textnormal{tr}} #1}
\DeclareMathOperator{\Tr}{trace}
\newcommand{\vspan}[1]{\mathop{\textnormal{span}}\{#1\}}
\newcommand{\diag}[1]{\mathop{\textsf{diag}} #1}
\newcommand{\DIAG}[1]{\mathop{\textnormal{DIAG}} #1}
\newcommand{\rank}[1]{\mathop{\textnormal{rank}} #1}
\newcommand{\mv}[1]{\mathbf{#1}}

%%% ==== Theorems and stuff
%\iffalse
\theoremstyle{plain}                   % default
\newtheorem{thm}{Theorem}[section]
\newtheorem{lmm}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}

\theoremstyle{definition}              % Examples and all
\newtheorem{pbm}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{opm}{Open Problem}
\newtheorem{conj}{Conjecture}
\newtheorem{ex}{Example}
\newtheorem{exer}{Exercise}
\newtheorem{defn}{Definition}
\newtheorem{alg}{Algorithm}
\newtheorem{rmk}{Remark}
\newtheorem{claim}{Claim}
\newtheorem{fact}{Fact}
%\newtheorem*{note}{Note}
%\fi

\definecolor{Red}{RGB}{255,204,204}
\definecolor{Green}{RGB}{204,255,204}
\definecolor{Blue}{RGB}{204,204,255}

%\allowdisplaybreaks
%\usepackage{acmart}

% the following is to prevent references in section headings from capitalization
\usepackage{xpatch}
\usepackage{textcase}
\makeatletter
\xpatchcmd{\@sect}{\uppercase}{\MakeTextUppercase}{}{}
\xpatchcmd{\@sect}{\uppercase}{\MakeTextUppercase}{}{}
\makeatother

%\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}
% To turn off hyperref "Token not allowed" warnings,
% add "bookmarks=false" to the above hyperref options

\allowdisplaybreaks[1]
\renewcommand{\vec}[1]{\ensuremath\boldsymbol{#1}}
\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}

%%%% Proceedings format for most of ACM conferences (with the exceptions listed below) and all ICPS volumes.
%\documentclass[sigconf]{acmart}

\usepackage{booktabs} % For formal tables


